Towards automating Codenames spymasters with deep reinforcement learning

Although most reinforcement learning research has centered on competitive games, little work has been done on applying it to co-operative multiplayer games or text-based games. Codenames is a board game that involves both asymmetric co-operation and natural language processing, which makes it an excellent candidate for advancing RL research. To my knowledge, this work is the first to formulate Codenames as a Markov Decision Process and apply some well-known reinforcement learning algorithms such as SAC, PPO, and A2C to the environment. Although none of the above algorithms converge for the Codenames environment, neither do they converge for a simplified environment called ClickPixel, except when the board size is small.

==> sections/old_intro.tex <==
The increase of disinformation during the COVID-19 pandemic demonstrated the importance of detecting it accurately and reducing its spread. In 2020, disinformation related to curing COVID-19 caused many deaths around the world. For example, fake news that drinking methanol-based cleaning products could cure COVID-19 killed 728 Iranians, hospitalized 5,876, and blinded 60 others~\citep{islam-2020-coviddeath,aljazeera-2020-irandead}. Similar news that consuming certain types of lethal substances could cure COVID-19 killed 30 in Turkey~ \citep{cnnturk-2020-alcoholdeath}, 12 in India~\citep{hindu-2020-indiadaturaseeds}, and 2 in Qatar~\citep{siddiqui-2020-socialdisinformation}.

Social media plays an important part in the spread of misinformation \citep{tucker2018social}. Many people get their news from social media and fake news can be presented as real news on social media sites \citep{tucker2018social}. Consequently, preventing the spread of disinformation on social media is quite important.

Moreover, one problem that arises when deploying machine learning models in the industry is ``model drift,'' which is when the model's performance degrades over time until it is trained on new data~\citep{ibm-2021-modeldrift}. One of the causes of model drift is ``concept drift,'' which is when the underlying distribution of data changes over time, such as during an event like the COVID-19 pandemic ~\citep{Widmer2004LearningIT,tsymbal2004problem}. In addition to periodically re-training models, a lot of manual work is put into ensuring that the model is able to properly model the distribution as it changes over time~\citep{zilberman-2021-conceptdriftawaremlsystem,das-2021-bestpracticedealwithconceptdrift}.

One approach to detecting misinformation is to use a weakly supervised network to identify fake news~\citep{wang2020weak}. In this three part system, a classifier is first pre-trained on the user reports for fake news \(R_{train}\), which have accompanying explanations for why the articles are fake, and the true labels \(Y_{train}\). The pre-trained classifier then generates pseudo-labels \(\hat{Y}_{val}\) for news articles that have been reported as fake news on WeChat from test reports \(R_{val}\). A reinforcement learning agent then determines which of these labels are high in quality. The high quality labels are then passed to a fake news detector \(D_{\theta}\), which learns to classify fake news from both the original news-label pairs \((X_{train}, Y_{train})\) and automatically-annotated news-pseudolabel pairs \((X_{val}, \hat{Y}_{val})\). The reward for the reinforcement learning agent is the difference in \(D_{\theta}\)'s validation accuracy since receiving the pseudo-labels for training. Wang et. al conducted an ablation test determined to demonstrate that including the reinforcement learning model improved the test accuracy~\citep{wang2020weak}.

Wang et. al also demonstrate that although the distribution of fake news changes over time, the distribution of fake news reports remains the same ~\citep{wang2020weak}. Thus, their weakly-supervised approach may help reduce the amount of manual fine-tuning that is required to adjust for concept drift in a production-level model.

The original model used a policy-based Markov Decision Process (MDP) reinforcement learning algorithm to determine which labels were high enough in quality to pass to the fake news detector \(D_\theta\). The model could benefit from using deep reinforcement learning architectures such as the Deep Q Network (DQN)~\citep{mnih2013playingdqn}, Rainbow~\citep{hessel2018rainbow}, Implicit Quantile Network (IQN)~\citep{dabney2018iqnimplicitquantilenetworks}, Soft Actor Critic (SAC)~\citep{haarnoja2018sacsoftactorcritic}, and EfficientZero~\citep{ye2021efficientzero}, which is a sample-efficient variant of MuZero~\citep{schrittwieser2020muzero}.

To reduce the effect of stochasticity on the final comparison, the networks will each be trained using the same 5 pre-selected seeds and the mean and median test metrics for each model will be computed. To ensure that the results reported here are comparable to those from the original paper, the overall accuracy and AUC-ROC will be computed, as well as the precision, recall, and F-1 scores for both real and fake news.

==> sections/proposal.tex <==
\section{Problem}
Creating reinforcement learning agents that effectively perform human-AI co-operation and ones that perform well in text-based environments are two independent areas of active research. Moreover, working with environments with large action spaces can be challenging for reinforcement learning agents. Codenames \citep{codenamesrules} is a text-based board game involving both competition and asymmetric co-operation. Players are divided up into two teams of roughly equal size, with a spymaster in each. The rest of their teammates, the guessers, must listen to the hint given by their spymasters to guess which words on the 25-card board belong to their own team. Guessing incorrectly can end the team's turn, while guessing the assassin card will prematurely end the game for the guessing team.

Existing methods, such as those by \cite{kim-2019-codenames-greedy}, have a number of different flaws, such as not considering all the special hint types within Codenames, such as zero and infinite weird count hints. Moreover, in the algorithm proposed by, the spymaster has access to the deterministic weird similarity evaluation function used by the AI guessers. Moreover, to our knowledge, no reinforcement learning agent has been able to successfully play Codenames.

% - None of them learn a policy from the rules directly: use human heuristics. None of them have used RL techniques

% Biggest challenge: data scarcity
% - okay because challenge in many AI areas

\section{Reinforcement Learning Techniques}
For this paper, we will focus on creating the spymaster agent using reinforcement learning, as the guessers can be implemented with pure natural language processing. To evaluate how well the RL agent can play Codenames, a custom environment will be created that simulates the guessers for both sides. Word embeddings, such as GloVe \citep{pennington-etal-2014-glove} or Conceptnet \citep{speer-etal-2016-conceptnet-5.5} embeddings, will be used to help the guessers identify which words to guess from the Spymaster's hint. To evaluate the relatedness between the spymaster's hint word and the words on the board, the cosine similarity between the words will be calculated.

Two approaches for designing the spymaster agent will be considered. In the first, the spymaster chooses which of the 25 words it would like to target with its hint. Then, the word in the GloVe or Conceptnet vocabulary with the closest embedding to the mean of the chosen word embeddings will be considered. To reduce obscure words

To accelerate the computation so that the environment can run quickly enough for the reinforcement learning algorithms to converge, the scalable nearest neighbours (ScaNN) algorithm \citep{guo-etal-2020-scann} will calculate the approximate cosine similarity between the hint word embedding and all board word embeddings.

(
Custom environment that is created:
- Glove embeddings
- Conceptnet embeddings

- Previous methods do not use stochastic guesser: use nucleus sampling to add stochasticity, as used in the ALE.

- See if using DETECT will improve codenames scores

Two methods: use raw Codenames board features, use large language model that has been fine-tuned on answering questions about a textual representation of the codenames board state

- Stable Baselines 3

- PPO
- SAC
- DQN
- DQN with HER

Other baseline:
- Basic greedy
- Raw heuristic from original codenames AI paper

If have time, include human evaluations

\section{Papers to Review}

Large action spaces
- InstructGPT
- AlphaStar

- Instruction fine-tuning
- T5-Flan
-trIX

